Local Stability and Stabilization of Quadratic-Bilinear Systems using Petersen's Lemma

Quadratic-bilinear (QB) systems arise in many areas of science and engineering. In this paper, we present a scalable approach for designing locally stabilizing state-feedback control laws and certifying the local stability of QB systems. Sufficient conditions are established for local stability and stabilization based on quadratic Lyapunov functions, which also provide ellipsoidal inner-estimates for the region of attraction and region of stabilizability of an equilibrium point. Our formulation exploits Petersen's Lemma to convert the problem of certifying the sign-definiteness of the Lyapunov condition into a line search over a single scalar parameter. The resulting linear matrix inequality (LMI) conditions scale quadratically with the state dimension for both stability analysis and control synthesis, thus enabling analysis and control of QB systems with hundreds of state variables without resorting to specialized implementations. We demonstrate the approach on three benchmark problems from the existing literature. In all cases, we find our formulation yields comparable approximations of stability domains as determined by other established tools that are otherwise restricted to systems with up to tens of state variables.

==> mainresult_old.tex <==
\section{Local Stability Analysis of Quadratic Systems}
\label{sec:analysis}
Our objective is to determine an ellipsoidal estimate  for the ROA of the quadratic system~\eqref{eq:quad}.

%
To do so, consider the quadratic Lyapunov function
\begin{equation}
    V(x) = x^\top Q x, \quad Q \succ 0.
    \label{eq:lyapunov_function}
\end{equation}

An expression for $\dot{V}(x)$ along trajectories of the quadratic system can be obtained by combining \eqref{eq:lyapunov_function},  \eqref{eq:quad}, and \eqref{eq:expandquad} as

\begin{align} 
    \dot{V}(x) &= \dot{x}^\top Q x + x^\top Q \dot{x} \nonumber \\
               &= \left(A x + H (x \otimes x)\right)^\top Q x + x^\top Q \left(A x + H (x \otimes x)\right) \nonumber \\
               &= \left(A x + \sum_{i=1}^n H_i x e_i^\top x \right)^\top Q x  + x^\top Q \left(A x + \sum_{i=1}^n H_i x e_i^\top x \right) \nonumber \\
               &= x^\top A^\top Q x + \left( \sum_{i=1}^n x^\top e_i x^\top H_i^\top \right) Q x 
                + x^\top Q A x + x^\top Q \sum_{i=1}^n H_i x e_i^\top x \nonumber \\
               &= x^\top \bigg( A^\top Q + Q A + \sum_{i=1}^n \Big( e_i x^\top H_i^\top Q + Q H_i x e_i^\top \Big) \bigg) x.
    \label{eq:Vdot}
\end{align}

For \( \dot{V}(x) < 0 \), we require
%

\begin{equation}
    A^T Q + Q A + \sum_{i=1}^n e_i x^T H_i^T Q + Q \sum_{i=1}^n H_i x e_i^T \prec 0.
    \label{eq:lyapunov_condition}
\end{equation}
%
Pre- and post-multiplying the inequality in~\eqref{eq:lyapunov_condition} by \( P = Q^{-1} \succ 0 \), we arrive at the equivalent condition
\begin{align}
    P A^T + A P &+ P \sum_{i=1}^n e_i x^T H_i^T 
    + \sum_{i=1}^n H_i x e_i^T P 
    \prec 0.
    \label{TT}
\end{align}

We are now ready to state our main analysis result as Theorem~\ref{thm:main_analysis}.
\begin{theorem}
\label{thm:main_analysis}
    Let \( \varepsilon > 0 \) be given. If \( P \succ 0 \) is a solution to the linear matrix inequality
    \begin{equation}
            \begin{bmatrix}
        AP + PA^\top + \varepsilon \sum_{i=1}^{n} H_i P H_i^\top  & P \\
        P & -\varepsilon I
    \end{bmatrix} \prec 0,
    \label{eq:lmi}
    \end{equation}
     then
    \begin{equation}        
\label{eq:ellipsoid}    \ehat = \left\{ x \in \mathbb{R}^n \ \bigg| \ x^\top P^{-1} x \leq 1 \right\}
    \end{equation}
    is an ellipsoidal approximation of the ROA for the quadratic system \eqref{eq:quad}, and     the quadratic form 
\begin{equation}
    V(x) = x^\top P^{-1} x
\end{equation}
    serves as a Lyapunov function for the system inside \( \ehat \).
\end{theorem}

\begin{pf}
We proceed to establish equivalence with the conditions of Lemma~\ref{lemma:roahat}, beginning with conditions 2(a) and 2(b) then ending with condition 1.
%

Condition 2(a) is satisfied by construction of the Lyapunov function~\eqref{eq:lyapunov_function}.
%

For condition 2(b), $\dot{V}(0)=0$ by construction as seen in~\eqref{eq:Vdot}.
%
To establish $\dot{V}(x)<0$ for all $x\in\ehat\backslash\{0\}$, we will make use of Petersen's Lemma.
%
First, let $\Delta =
    \begin{bmatrix}
          e_1x^T P^{-\frac{1}{2}}&
         e_2x^TP^{-\frac{1}{2}} & 
        \cdots & 
         e_nx^TP^{-\frac{1}{2}}
    \end{bmatrix}^T$.
%
Accordingly, $\Delta^T\Delta = \sum_{i=1}^ne_ix^TP^{-1}xe_i^T=x^TP^{-1}x$, and thus $\|\Delta\|_2\le1$ is equivalent to $x^TP^{-1}x\le1$.

%
Next, invoke Lemma~\ref{lemma:petersen} (Petersen's Lemma) with  $G = PA^T+AP$, $M = \begin{bmatrix}
        H_1P^{\frac{1}{2}}  & H_2P^{\frac{1}{2}}  & \cdots & H_nP^{\frac{1}{2}} 
    \end{bmatrix}$, $N = P$.
    %
It follows that \eqref{TT} holds for all $x\in\ehat$
if and only if there exists a scalar $\varepsilon > 0$ such that $G + \varepsilon M M^\top + \frac{1}{\varepsilon} N^\top N \prec 0$.
%
Applying the Schur Complement Lemma yields the desired condition~\eqref{eq:lmi}. 
%

Finally, condition 1 requires that $\ehat$ be an invariant set, which is satisfied by virtue of the fact that $\ehat$ is defined by the Lyapunov function level set $V(x)=x^TP^{-1}x\le1$ on which $\dot{V}(x)<0$.
%
Thus, all trajectories starting in $\ehat$ remain in $\ehat$ for all time, and asymptotically decay to the origin.
\qed
\end{pf}

Theorem~\ref{thm:main_analysis} establishes a means for determining an ellipsoidal approximation $\ehat \subseteq\roa$ of~\eqref{eq:quad} by performing a line search over $\varepsilon>0$.
%
For a given $\varepsilon>0$, the condition in~\eqref{eq:lmi} is an LMI feasibility condition.
%
As such, Theorem~\ref{thm:main_analysis} defines a family of ellipsoidal approximations.
%
It is possible to optimize over this family to obtain desirable properties for the approximation, usually maximizing its size in a some manner: e.g., maximizing the volume or the leading principal axis of $\ehat$.

Here, we seek an ellipsoidal approximation for which the sum of the squares of its principal axes is maximized: i.e., given $\varepsilon>0$,
%
%
    \begin{equation}    
    \max_{P\succ0} \quad \text{trace}(P) \quad \text{subject to~\eqref{eq:lmi}. } 
    \label{cor:trace}
    \end{equation}
   



The optimization in~\eqref{cor:trace} yields an ellipsoidal approximation $\ehat$ for a fixed value of $\varepsilon>0$.
%
A bisection can be performed over $\varepsilon$ to obtain the maximum such ellipsoidal approximation $\ehat^*$ with corresponding $\varepsilon=\varepsilon^*>0$.
%\end{rem}
In light of the discussions above on optimality, it is important to note the following:
Even if an optimal ellipsoidal approximation can be found, this approximation may not encapsulate the complete ROA, which in general may not be ellipsoidal.
%
It is possible to improve the ROA approximation by considering multiple ellipsoidal approximations~\cite{Chesi2007}.
%
Consider a collection of ellipsoidal approximations $\ehat_i$ with $i=1,\dots,M$ determined from pairs $(P_i,\varepsilon_i)$---not necessarily optimal---for which~\eqref{eq:lmi} holds.
%
Since $\ehat_i\subseteq\roa$, a more complete approximation of the ROA $\roa$ can be constructed as the union of these ellipsoidal approximations, i.e.,
\begin{equation}
        \roahat=\bigcup_{i=1}^M \ehat_i \subseteq \roa.
        \label{eq:union}
\end{equation}
Furthermore, the ROA approximation $\roahat$ constructed as in~\eqref{eq:union} will not necessarily be ellipsoidal nor even convex.

\begin{remark}
    The objective function is maximized under strict inequality constraints \eqref{eq:lmi}. To formulate and solve a well-posed problem, consider the nonstrict matrix inequality
    \begin{equation}
        PA^T + AP + \varepsilon \sum_{i=1}^n H_i P H_i^T + \frac{1}{\varepsilon} P^2 \preceq -\alpha P
        \label{eq:modifyLMI}
    \end{equation} 
    \msh{this is fine, but wasn't the right hand side previously set to $-\alpha I$? What did you implement when solving each of the example problems?}
    for some $\alpha > 0$, i.e., with a negative definite right-hand side. By the Schur Complement Lemma, inequality \eqref{eq:modifyLMI} can be represented in an equivalent form, linear in $P$:  
    \begin{equation}
        \label{eq:sdp_problem2}
        \begin{bmatrix}
            A P + P A^T + \varepsilon \sum_{i=1}^{n} H_i P H_i^\top + \alpha P & P \\
            P & -\varepsilon I
        \end{bmatrix}
        \preceq 0.
    \end{equation}
    Changing the first constraint in \eqref{eq:lmi} to this matrix inequality, and using ~\eqref{eq:Vdot},~\eqref{eq:modifyLMI}, and~\eqref{eq:Petersen}, we obtain
    \begin{align}
        \dot{V}(x) &= x^\top \left( A^\top Q + Q A + \sum_{i=1}^n \left( e_i x^\top H_i^\top Q + Q H_i x e_i^\top \right) \right) x \notag \\
        &= x^\top Q \left( P A^\top + A P + \sum_{i=1}^n \left( P e_i x^\top H_i^\top + H_i x e_i^\top P \right) \right) Q x \notag \\
        &\preceq x^\top Q \left( A P + P A^\top + \varepsilon \sum_{i=1}^n H_i P H_i^\top + \frac{1}{\varepsilon} P^2 \right) Q x \notag \\
        &\preceq x^\top Q \left( -\alpha P \right) Q x = -\alpha V(x).
        \label{eq:V_derivative}
    \end{align}
    
    Hence, the Lyapunov function decreases no slower than $e^{-\alpha t}$:
    \[
        V(x(t)) \leq V(x(0)) e^{-\alpha t}.
    \]
\end{remark}
Similar to the line search performed over \(\varepsilon\), we also perform a line search over \(\alpha > 0\) to maximize \(\text{trace}(P)\). This dual line search strategy allows us to optimize the ellipsoidal approximation \(\ehat\) by adjusting both parameters, ensuring that the trace of \(P\) is maximized for each fixed \(\varepsilon\). In practice, the parameters \(\varepsilon\) and \(\alpha\) are selected based on trial and error to fine-tune the approximation effectively.








\section{Stabilizing Controller Synthesis for Quadratic Bilinear Systems}
\label{sec:synthesis}
The analysis approach from Section~\ref{sec:analysis} can be extended to synthesizing stabilizing controllers.
%
Consider the QB system~\eqref{eq:qb} with the input determined by a static linear state feedback law as 
\begin{equation}
u = K x, \quad K \in \mathbb{R}^{m \times n}
\label{Controller}
\end{equation}
%
with \( m < n \).
%
Here, we seek a control gain $K$ that guarantees the closed-loop dynamics will be stable within an ellipsoid centered about the origin.
%
To this end, we express the associated closed-loop dynamics as
\begin{equation}
    \dot{x} = (A + B K) x + \sum_{i=1}^n \begin{bmatrix} H_i & D_i \end{bmatrix}
    \begin{bmatrix} 
        x e_i^\top & 0 \\ 
        0 & x e_i^\top 
    \end{bmatrix}
    \begin{bmatrix} 
        I \\ 
        \tilde{K} 
    \end{bmatrix} x
    \label{eq:quad_feedback}
\end{equation}
where we have defined
\begin{align}
    D_i &:= 0 \quad \text{for } i = m+1, \dots, n, \\
    \tilde{K} &:= \begin{bmatrix}
        K \\
        0
    \end{bmatrix} \in \mathbb{R}^{n \times n}.
\end{align}

Next, introduce a quadratic Lyapunov function~\eqref{eq:lyapunov_function}: i.e., $V(x)=x^TQx$ with $Q \succ 0$.
%
It follows from~\eqref{eq:lyapunov_function} and \eqref{eq:quad_feedback} that 
\begin{align}
    \dot{V}(x) &= \dot{x}^T Q x + x^T Q \dot{x} \nonumber \\
    & = x\left((A+BK)^TQ + Q(A+BK)   + Q\sum_{i=1}^n 
      \begin{bmatrix}
          H_i & D_i
      \end{bmatrix}
      \begin{bmatrix}
          xe_i^T & 0 \\
          0 & xe_i^T
      \end{bmatrix}
      \begin{bmatrix}
          I \\ \tilde{K} 
      \end{bmatrix}  + \sum_{i=1}^n 
      \begin{bmatrix}
           I & \tilde{K}^T 
      \end{bmatrix}
      \begin{bmatrix}
          xe_i^T & 0 \\
          0 & xe_i^T
      \end{bmatrix}^T
      \begin{bmatrix}
          H_i^T \\ 
          D_i^T
      \end{bmatrix}Q\right)x  < 0.
    
  \label{eq:VdotCL}
\end{align}
%
For \( \dot{V}(x) < 0 \), we require
\begin{align*}
    & & (A+BK)^TQ + Q(A+BK)   + Q\sum_{i=1}^n 
      \begin{bmatrix}
          H_i & D_i
      \end{bmatrix}
      \begin{bmatrix}
          xe_i^T & 0 \\
          0 & xe_i^T
      \end{bmatrix}
      \begin{bmatrix}
        I \\  \tilde{K}  
      \end{bmatrix}  + \sum_{i=1}^n 
      \begin{bmatrix}
         I & \tilde{K}^T 
      \end{bmatrix}
      \begin{bmatrix}
          xe_i^T & 0 \\
          0 & xe_i^T
      \end{bmatrix}^T
      \begin{bmatrix}
          H_i^T \\ 
          D_i^T
      \end{bmatrix}Q  \prec 0.
\end{align*}
%
Pre- and post-multiplying the inequality above by the matrix \( P = Q^{-1} \succ 0 \) yields the equivalent condition
\begin{align}
    & P(A+BK)^T + (A+BK) P  + \sum_{i=1}^n 
      \begin{bmatrix}
          H_i & D_i
      \end{bmatrix}
      \begin{bmatrix}
          xe_i^T & 0 \\
          0 & xe_i^T
      \end{bmatrix}
      \begin{bmatrix}
         P \\ \tilde{K} P 
      \end{bmatrix}  + \sum_{i=1}^n 
      \begin{bmatrix}
          P & P \tilde{K}^T 
      \end{bmatrix}
      \begin{bmatrix}
          xe_i^T & 0 \\
          0 & xe_i^T
      \end{bmatrix}^T
      \begin{bmatrix}
          H_i^T \\ 
          D_i^T
      \end{bmatrix}  \prec 0.
    \label{LMi3}
\end{align}
%\msh{note that the terms with $KP$ show up in an inconsistent order with the rest (starting from above). Let's fix this to make it look ``more beautiful''.  The parantheses only need to be included in the last version here, but perhaps could be useful to add in (26) above as well.  }
%
%Note that we have two pairs of summations in~\eqref{eq:multiunc}---one pair over $j=1,\dots,m$ and the other pair over $i=1,\dots,n$---which will result in two distinct uncertainties $\Delta_1$ and $\Delta_2$, which in principle can be accommodated using a generalized Petersen's lemma~\cite{Khlebnikov2008}.
%
%However, the generalized Petersen's lemma over multiple distinct uncertainties only provides a sufficient condition for the sign-definiteness of~\eqref{eq:multiunc} due to the distinct factors $P$ and $KP$ between them, and therefore may yield conservative results (see~\cite{Khlebnikov2008}).
%
%To obtain an equivalent representation that can be used directly with Petersen's Lemma (Lemma~\ref{lemma:petersen})---and thus a necessary and sufficient condition for the sign definiteness of~\eqref{eq:multiunc}---define 
%\begin{align}
 %   D_j&:=0 \text{ for } j=m+1,\dots,n\\
  %  \tilde{K} &:= \begin{bmatrix}
  %      K^T & 
    %    0
%\end{bmatrix}^T\in\mathbb{R}^{n\times n}
%\end{align}
%such that $\sum_{j=1}^m D_j x f_j^T K P = \sum_{j=1}^n D_j x e_j^T \tilde{K} P$.
%
% So, we can rewrite the inequality as:
% \begin{align}
%     & PA_c^T + A_c P  + \sum_{i=1}^n D_i x e_i^T \tilde{K} P  + \sum_{i=1}^n P \tilde{K}^T e_i x^T D_i^T  + \sum_{i=1}^n P e_i x^T H_i^T  + \sum_{i=1}^n H_i x e_i^T P \prec 0,
%     \label{LMi2}
% \end{align}

% where \( D_i = 0 \) for \( i > j \), and \( \tilde{K} \) is defined as:
% \[
%     \tilde{K} = \begin{bmatrix}
%         K \\ 
%         0
%     \end{bmatrix}.
% \]
% Then, we can rewrite the inequality as follows:
%Thus, \eqref{eq:multiunc} can be re-expressed in a form that allows for direct application of Lemma~\ref{lemma:petersen} (Petersen's lemma):


We are now ready to state our main synthesis result as Theorem~\ref{thm:main_synthesis}.



\begin{theorem}
    \label{thm:main_synthesis}
    Let $\varepsilon>0$ be given.
    %
    If $P\succ0$ and $Y\in\mathbb{R}^{m \times n}$ satisfy the LMI 
\begin{align}
\left[
\begin{array}{c|c}
    A P + P A^\top + B Y + Y^\top B^\top + \varepsilon \sum_{i=1}^{n} H_i P H_i^\top + \varepsilon \sum_{j=1}^{m} D_j P D_j^\top &\quad P \quad \begin{bmatrix} Y \\ 0 \end{bmatrix} \\
    \hline 
    P \\ \begin{bmatrix}
        Y^\top & 0
    \end{bmatrix} & -\varepsilon I
\end{array}
\right] 
\prec 0,
\label{eq:sdp_problem}
\end{align}
then the linear state feedback gain
\[
K = YP^{-1} 
\]
stabilizes the QB system~\eqref{eq:qb} inside the ellipsoid
\[
\hat{\mathcal{E}} = \{ x \in \mathbb{R}^n : x^T P^{-1} x \leq 1 \},
\]
and the quadratic form
\[
V(x) = x^T P^{-1} x
\]
is a Lyapunov function for the closed-loop system inside the ellipsoid \(\hat{\mathcal{E}}\).
\end{theorem}

\msh{Theorem 2 reduces to Theorem 1 when $D=0$, $B=0$, $K=0$ ($K=0\implies Y=0$.  Perhaps this is the way to tell the story. We were originally trying to find a way to prove Thm 2 from Thm 1, but we missed that we can easily arrive at Thm 1 from Thm 2.}

\begin{pf}
We proceed to establish equivalence with the conditions of Lemma~\ref{lemma:roahat} for the closed-loop QB system~\eqref{eq:quad_feedback}, beginning with conditions 2(a) and 2(b) then ending with condition 1.

Condition 2(a) is satisfied by construction of the Lyapunov function~\eqref{eq:lyapunov_function}.
%

For condition 2(b), $\dot{V}(0)=0$ by construction as seen in~\eqref{eq:VdotCL}.
%
To establish $\dot{V}(x)<0$ for all $x\in\ehat\backslash\{0\}$, we will make use of Petersen's Lemma.
%
First, let $\Delta =
    \begin{bmatrix}
          I_2 \otimes  e_1x^T P^{-\frac{1}{2}},&
         I_2 \otimes  e_2x^TP^{-\frac{1}{2}}, & 
        \cdots, & 
         I_2 \otimes  e_nx^TP^{-\frac{1}{2}}
    \end{bmatrix}^T$, where $I_2\in\mathbb{R}^{2\times 2}$ is the identity matrix.
%
Accordingly, $\Delta^T\Delta = \sum_{i=1}^n \left(I_2 \otimes  e_ix^T P^{-\frac{1}{2}}\right)\left(I_2 \otimes   P^{-\frac{1}{2}}xe_i^T\right)=\sum_{i=1}^n (I_2)\otimes\left(e_ix^TP^{-1}xe_i^T\right)=(I_2)\otimes\left(x^TP^{-1}x\right)$, and thus $\|\Delta\|_2\le1$ is equivalent to $x^TP^{-1}x\le1.$
%
% By Lemma~\ref{lemma:spectral_norm_block_diag}\msh{should update Lemma to accommodate this more general structure}, $\|\Delta\|^2_2=x^TP^{-1}x$.
%
Next, invoke Lemma~\ref{lemma:petersen} (Petersen's Lemma) with  $G = P(A+BK)^T+(A+BK)P$, $M  = \begin{bmatrix}
    D_1 P^{\frac{1}{2}} \quad H_1 P^{\frac{1}{2}} & 
    D_2 P^{\frac{1}{2}} \quad H_2 P^{\frac{1}{2}} & 
    \cdots & 
    D_n P^{\frac{1}{2}} \quad H_n P^{\frac{1}{2}}
\end{bmatrix}$, and $N = \begin{bmatrix}
        P\tilde{K}^T&
        P
    \end{bmatrix}^T$.
%
It follows that \eqref{LMi3} holds for all $x\in\ehat$
if and only if there exists a scalar $\varepsilon > 0$ such that $G + \varepsilon M M^\top + \frac{1}{\varepsilon} N^\top N \prec 0$.
%
For $\epsilon>0$ given, defining $Y:=KP$, applying the Schur Complement Lemma, and noting that $D_j=0$ for $j=m+1,\dots,n$ yields 
the desired LMI condition~\eqref{eq:sdp_problem}.
%
The control gain $K=YP^{-1}$ can be uniquely determined since $P\succ0$.

Finally, condition 1 requires that $\ehat$ be an invariant set, which is satisfied by virtue of the fact that $\ehat$ is defined by the Lyapunov function level set $V(x)=x^TP^{-1}x\le1$ on which $\dot{V}(x)<0$. \qed

%     Similarly to the analysis procedure, we perform the synthesis by invoking Petersen's Lemma on equation~\eqref{LMi3}, with the matrices \( G \), \( M \), \( N \), and \( \Delta \) defined as follows:

% \begin{align}
%     G &= P A_c^\top + A_c P, \label{G_definition} \quad M  = \begin{bmatrix}
%     D_1 P^{\frac{1}{2}} \quad H_1 P^{\frac{1}{2}} & 
%     D_2 P^{\frac{1}{2}} \quad H_2 P^{\frac{1}{2}} & 
%     \cdots & 
%     D_n P^{\frac{1}{2}} \quad H_n P^{\frac{1}{2}}
% \end{bmatrix}, \nonumber \\
%     N &= \begin{bmatrix}
%         \tilde{K} P \\
%         P
%     \end{bmatrix} \label{N_definition} , \quad  \Delta = \begin{bmatrix}
%         I_2 \otimes P^{-\frac{1}{2}} x e_1^\top \\  
%         I_2 \otimes P^{-\frac{1}{2}} x e_2^\top \\ 
%         \vdots \\  
%         I_2 \otimes P^{-\frac{1}{2}} x e_n^\top
%     \end{bmatrix} \label{Delta_definition} 
% \end{align}
%     And by lemma 2 which norm of $\Delta$ will be $x^TP^{-1}x$ and introduce an auxiliary vector variable $PK = Y$. Since \( P \succ 0 \), the vector \( K \) can be uniquely recovered as \( K = P^{-1}Y \) and obtain a linear matrix inequality. 

\end{pf}


% \begin{rem}
% \label{rem:family_feedback}
For a given \(\varepsilon > 0\), the condition \eqref{eq:sdp_problem} is an LMI feasibility condition. As such, Theorem~\ref{thm:main_synthesis} defines a family of ellipsoidal approximations over which we can optimize.  
%
As in the context of analysis, many choices can be made for the objective function in this optimization.
%
Here again we seek to stabilize the system within an ellipsoid for which the sum of the squares of its principal axes is maximized: i.e., given $\varepsilon>0$,
   \begin{equation}    
    \max_{P\succ0,Y} \quad \text{trace}(P) \quad \text{subject to~\eqref{LMi3} } 
    \label{cor:largest_stabilizability_ellipsoid}
    \end{equation}
%\end{rem}
from which the optimal controller gain $K=YP^{-1}$ can be determined.
%
The associated ellipsoidal estimate for the ROA of the closed-loop system~$\ehat$ is sometimes referred to as a \emph{stabilizability ellipsoid}~\cite{Khlebnikov2015,Khlebnikov2017}.  The stabilizability ellipsoid provides an approximation of the region of stabilizability~(ROS)---i.e.,~the region of state-space for which there exists a stabilizing controller to asymptotically steer the system from any state within this region to the origin.
%
We note that the stabilizing controller need not be the same for all points within the ROS.

% \begin{Corollary}
% \label{cor:largest_stabilizability_ellipsoid}
% Under the conditions of Theorem \ref{thm:main_synthesis}, the largest stabilizability ellipsoid \(\ehat\) is obtained by solving the optimization problem:
% \[
% \max \quad \text{trace}(P)
% \]
% subject to the matrix inequality:

% \begin{align*}
% \left[
% \begin{array}{c|c}
%     A P + P A^\top + B Y + Y^\top B^\top + \varepsilon \sum_{i=1}^{n} \left( H_i P H_i^\top + D_i P D_i^\top \right) &\quad P \quad \begin{bmatrix} Y \\ 0 \end{bmatrix} \\
%     \hline 
%     P \\ \begin{bmatrix}
%         Y^\top & 0
%     \end{bmatrix} & -\varepsilon I
% \end{array}
% \right] 
% \prec 0,
% \label{eq:sdp_problem}
% \end{align*}

% where \( P \succ 0 \), \(\varepsilon > 0\). The resulting gain matrix is \( K = P^{-1} Y \), and the ellipsoid
% \[
% \ehat = \left\{ x \in \mathbb{R}^n \ \bigg| \ x^\top P^{-1} x \leq 1 \right\}
% \]
% is the largest ellipsoid within which the quadratic bilinear system \eqref{eq:qb} is guaranteed to be stabilized by the linear feedback controller \( u = Kx \).
% \end{Corollary}

% \begin{rem}
% \label{rem:optimize_feedback}
The optimization in~\eqref{cor:largest_stabilizability_ellipsoid} yields an ellipsoidal approximation \(\ehat\) for a fixed value of \(\varepsilon > 0\). A bisection method can be applied to obtain the maximum stabilizability ellipsoid \(\ehat^*\) with corresponding \(\varepsilon = \varepsilon^* > 0\) and $K^*=Y^*(P^*)^{-1}$.
%
As in the analysis case, the union of stabilizability ellipsoids can provide a more complete approximation of the ROS as
\begin{equation}
    \roahat = \bigcup_{i=1}^M \ehat_i \subseteq \roa.
    \label{eq:union_stability_domains}
\end{equation}

% \begin{rem}
% Consider a collection of ellipsoidal approximations \(\ehat_i\) with \(i=1,\dots,M\) determined from triples \((K_i, P_i, \varepsilon_i)\)—not necessarily optimal—for which the matrix inequality \eqref{eq:sdp_problem} holds. Since each \(\ehat_i\) is a stability domain, meaning there exists a controller \(K_i\) that can stabilize the system within \(\ehat_i\), and \(\ehat_i \subseteq \mathcal{R}\), a more comprehensive approximation of the Region of Attraction \(\mathcal{R}\) can be constructed as the union of these stability domains, i.e.,
% \begin{equation}
%     \widehat{\mathcal{R}} = \bigcup_{i=1}^M \ehat_i \subseteq \mathcal{R}.
%     \label{eq:union_stability_domains}
% \end{equation}
% Furthermore, the ROA approximation \(\widehat{\mathcal{R}}\) constructed as in \eqref{eq:union_stability_domains} will not necessarily be ellipsoidal nor even convex.
% \end{rem}



\begin{rem}
     The objective function
is maximized under strict inequality constraints \eqref{eq:sdp_problem}; to formulate and solve a well-posed
problem, consider the nonstrict matrix inequality

\begin{equation}
   AP+PA^T+BY+Y^TB^T+\varepsilon \sum_{i=1}^n H_iPH_i^T+\varepsilon\sum_{j=1}^mD_jPD_j^T+\frac{1}{\varepsilon}  \begin{bmatrix}
        P\tilde{K}^T  & P
    \end{bmatrix}  \begin{bmatrix}
        \tilde{K} P \\
        P
    \end{bmatrix} \preceq -\alpha I
    \label{10}
\end{equation}
\msh{see my comment for remark 1. same question here.}
for some $\alpha > 0$, i.e., with a negative definite right-hand side. By Schur Complement Lemma, inequality \eqref{10} can
be represented in the equivalent form, linear in P

\begin{align}
\left[
\begin{array}{c|c}
    A P + P A^\top + B Y + Y^\top B^\top + \varepsilon \sum_{i=1}^n H_iPH_i^T+\varepsilon\sum_{j=1}^mD_jPD_j^T + \alpha I &\quad P \quad \begin{bmatrix} Y \\ 0 \end{bmatrix} \\
    \hline 
    P \\ \begin{bmatrix}
        Y^\top & 0
    \end{bmatrix} & -\varepsilon I
\end{array}
\right] 
\preceq 0.
\end{align}
\end{rem}
